Sparse Support Recovery with Non-smooth Loss Functions

In this paper, we study the support recovery guarantees of underdetermined sparse regression using the $\ell_1$-norm as a regularizer and a non-smooth loss function for data fidelity. More precisely, we focus in detail on the cases of $\ell_1$ and $\ell_\infty$ losses, and contrast them with the usual $\ell_2$ loss. While these losses are routinely used to account for either sparse ($\ell_1$ loss) or uniform ($\ell_\infty$ loss) noise models, a theoretical analysis of their performance is still lacking. In this article, we extend the existing theory from the smooth $\ell_2$ case to these non-smooth cases. We derive a sharp condition which ensures that the support of the vector to recover is stable to small additive noise in the observations, as long as the loss constraint size is tuned proportionally to the noise level. A distinctive feature of our theory is that it also explains what happens when the support is unstable. While the support is not stable anymore, we identify an "extended support" and show that this extended support is stable to small additive noise. To exemplify the usefulness of our theory, we give a detailed numerical analysis of the support stability/instability of compressed sensing recovery with these different losses. This highlights different parameter regimes, ranging from total support stability to progressively increasing support instability.

==> gfx/support_excess_phase_transition_fm <==
% fmopt: width=18cm
% head:
% \usepackage{amsmath,amssymb}
% end head


\psfrag{k}[c][u]{$k$}
\psfrag{al}[r][c]{$\dfrac{1}{\alpha}$}
\psfrag{se=0}[c][c]{$s_e = 0$}
\psfrag{se=50}[c][c]{$s_e = 50$}
\psfrag{se=150}[c][c]{$s_e = 150$}

\psfrag{1.0}[c][c]{$1$}
\psfrag{0.9}[c][c]{}
\psfrag{0.8}[c][c]{}
\psfrag{0.7}[c][c]{}
\psfrag{0.6}[c][c]{}
\psfrag{0.5}[c][c]{$0.5$}
\psfrag{0.4}[c][c]{}
\psfrag{0.3}[c][c]{}
\psfrag{0.2}[c][c]{}
\psfrag{0.1}[c][c]{}
\psfrag{0.0}[c][c]{$0$}

\psfrag{125}[c][c]{$125$}
\psfrag{250}[c][c]{$250$}
\psfrag{375}[c][c]{$375$}
\psfrag{500}[c][c]{$500$}

==> gfx/toy_example_2_fm <==
% fmopt: width=25cm
% head:
% \usepackage{amsmath,amssymb}
% end head


\psfrag{xtau}[c][u]{$x_\tau$}
\psfrag{eta}[c][c]{$\Phi^* p_\beta$}
\psfrag{x0}[c][c]{$x_0$}
\psfrag{xt1}[c][c]{$x_{\tau_1}$}
\psfrag{xt2}[c][c]{$x_{\tau_2}$}
\psfrag{Jc}[c][c]{$J_c$}
\psfrag{Jt}[c][c]{$\tilde{J}$}
\psfrag{I}[c][c]{$I$}
\psfrag{…}[c][c]{$\dots$}

\psfrag{1}[c][c]{$1$}
\psfrag{0}[c][c]{$0$}
\psfrag{-1}[c][c]{$-1$}


==> gfx/toy_example_compact_fm <==
% fmopt: width=19cm
% head:
% \usepackage{amsmath,amssymb}
% end head


\psfrag{xtau}[c][u]{$x_\tau$}
\psfrag{eta}[c][c]{$\Phi^* p_\beta$}
\psfrag{x0}[c][c]{$x_0$}
\psfrag{xt1}[c][c]{$x_{\tau_1}$}
\psfrag{xt2}[c][c]{$x_{\tau_2}$}
\psfrag{Jc}[c][c]{\small$J_c$}
\psfrag{Jt}[c][c]{\small$\tilde{J}$}
\psfrag{I}[c][c]{\small$I$}
\psfrag{…}[c][c]{$\dots$}

\psfrag{1}[c][c]{$1$}
\psfrag{0}[c][c]{$0$}
\psfrag{-1}[c][c]{$-1$}


==> gfx/transition_l1_l2_linf_fm <==
% fmopt: width=18cm
% head:
% \usepackage{amsmath,amssymb}
% end head

 
\psfrag{xlabel}[c][u]{$k$}
\psfrag{ylabel1}[c][c]{$\mathbb{P}[|\tilde{J}_{p_\infty}|\leqslant s_e]$}
\psfrag{ylabel2}[c][c]{$\mathbb{P}[|\tilde{J}_{p_2}| \leqslant s_e]$}
\psfrag{ylabelinf}[c][c]{$\mathbb{P}[|\tilde{J}_{p_1}| \leqslant s_e]$}
\psfrag{linf}[c][u]{$\ell_\infty$}
\psfrag{l2}[c][u]{$\ell_2$}
\psfrag{l1}[c][u]{$\ell_1$}

\psfrag{0}[c][c]{$0$}
\psfrag{1}[c][c]{$1$}

\psfrag{200}[c][c]{$200$}
\psfrag{400}[c][c]{$400$}
\psfrag{600}[c][c]{$600$}

==> sections/background.tex <==
% !TEX root = nips_2016.tex

\subsection{Identifiability}
An important assumption is that $x_0$ is a solution of \emph{Basis Pursuit} (BP) \cite{Chen1998}, 
\eql{
\label{BP}
\tag{$\Pp^0(\Phi x_0)$}
\umin{x} \ensst{\norm{x}_1 }{\Phi x = \Phi x_0},
}
\ie $x_0 \in \Argmin \eqref{BP}$. In that case, we say that $x_0$ is \emph{identifiable}. Note that BP is equivalent to \mbox{($\Pp_\al^\tau(\Phi x_0)$)} when $\tau = 0$. 


\subsection{Dual and saddle-point problems}

Using appropriately the Legendre transform, we find that the dual problem to~\eqref{primal-l1-lal} in the sense of Fenchel-Rockafellar \cite{Rockafellar} reads
\eql{
\tag{${\cal D}_\be^\tau(y)$}
\label{dual-l1-lbe}
	\umax{p} \ensst{ \dotp{y}{p} - \tau \norm{p}_\be }{ \norm{\Phi^* p}_{\infty} \leq 1 },
}
where $\norm{\cdot}_\be$ is the H\"{o}lder dual of the  \ellnorm{\al} with $\frac{1}{\al}+\frac{1}{\be}=1$.
The corresponding saddle point problem reads
\eql{
	\label{saddle-l1-lbe}
	\tag{${\cal S}_\be^\tau(y)$}
	\umin{x} \umax{p} \norm{x}_1 - \dotp{\Phi x}{p}  + \dotp{y}{p} - \tau \norm{p}_\be .
}
From the First Order (FO) optimality conditions, we deduce the first relationship for a primal-dual pair $(p,x)$,
\eq{
	\Phi^* p \in \partial \norm{x}_1,
}
which corresponds to the $\ell_1$ \textbf{r}egularization term and equivalently reads
\eql{\label{FOr}
	\tag{FO$_{\mbox{r}}$}
	\PhiI^* p = \sign(x_I)
	\qandq
	\norm{\Phi^* p}_\infty \leq 1.
}
Note that $\PhiI $ is the matrix $\Phi$ restricted to the columns indexed by $I$ and the dot indicates that we keep all the rows. Transposition is applied afterwards and we use this convention in the rest of the paper. 
The second relationship is specific to a particular choice of $\al$ for the \ellnorm{\al} data fidelity constraint and reads
\eql{\label{FObe}
	\tag{FO$_\be$}
	\frac{y - \Phi x}{\tau} \in \partial \norm{p}_\be.
}


\subsection{Dual certificates}
A vector $\bar{p} \in \RR^m$ is called a \emph{dual certificate} when the pair $(\bar{p},x_0)$ obeys \eqref{FOr}, that is, ${\Phi^* \bar{p} \in \partial \norm{x_0}_1}$, or
\eql{\label{eq-certif}
	%\tag{FO1}
	\PhiI^*\bar{p} = \sign(\xzI)
	\qandq
	\norm{\Phi^* \bar{p}}_\infty \leq 1.
}
When moreover, ${\norm{\PhiIc^* \bar{p}}_\infty < 1}$, the certificate is called \emph{non degenerate}. Note that as for \eqref{BP}, these definitions are independent of the data fidelity term. It can be verified, using the first order optimality conditions of \eqref{BP}, that 
the existence of a dual certificate is equivalent to $x_0$ being identifiable \cite{Fuchs2004}. Depending on the specific fidelity term used (here the value of $\al$), the support stability of the solution to \eqref{primal-l1-lal} is governed by a specific choice of $\bar{p}$.
%%%

\subsection{Minimum norm certificate} 
The certificates of minimum \ellnorm{\be} play an important role regarding support stability under small noise. They read
% as it comes from the asymptotic Fenchel dual of \eqref{primal-l1-lal} when ${\tau \rightarrow 0}$, \ie

\eqn{\label{eq-min-certif}
\tag{${\cal D}_{\be}^0(\Phi x_0)$}
	p_{\be} &\in \uArgmin{p} \ensst{\norm{p}_{\be} }{ \PhiI^* p = \sign(\xzI), \norm{\Phi^*p}_\infty \leq 1 }.
	\vspace{-5mm}
}

%where $\norm{\cdot}_\be$ is the dual \ellnorm{\be}, \ie $\frac{1}{\al}+\frac{1}{\be}=1$.
Since $\norm{\cdot}_\be$ is coercive, the existence of $\bar{p}$ implies the existence of $\pb$.
We also define $J_{p_\be}  \eqdef \sat(\Phi^* \pb)$, where $\sat(u) \eqdef \enscond{i}{|u_i|=\norm{u}_\infty} $ is the \emph{saturation support}. Non-degeneracy of $\pb$ is equivalent to $J_{p_\be}=I$.
Note that because $\be \in \{1,\infty\}$, the sublevel sets of $\norm{p}_{\be}$ are polyhedral and $\pb$ is not necessarily unique so that $J_{p_\be}$ actually depends on $\pb$. In order to simplify the notations, we will often omit the index and just write $J$, when it is clear from the context.
